On the (In)security of optimized Stern-like signature schemes

Stern's signature scheme is a historically important code-based signature scheme. A crucial optimization of this scheme is to generate pseudo-random vectors and a permutation instead of random ones, and most proposals that are based on Stern's signature use this optimization. However, its security has not been properly analyzed, especially when we use deterministic commitments. In this article, we study the security of this optimization. We first show that for some parameters, there is an attack that exploits this optimization and breaks the scheme in time $O(2^{\frac{\lambda}{2}})$ while the claimed security is $\lambda$ bits. This impacts in particular the recent Quasy-cyclic Stern signature scheme [BGMS22]. Our second result shows that there is an efficient fix to this attack. By adding a string $salt \in \{0,1\}^{2\lambda}$ to the scheme, and changing slightly how the pseudo-random strings are generated, we prove not only that our attack doesn't work but that for any attack, the scheme preserves $\lambda$ bits of security, and this fix increases the total signature size by only $2\lambda$ bits. We apply this construction to other optimizations on Stern's signature scheme, such as the use of Lee's metric or the use of hash trees, and we show how these optimizations improve the signature length of Stern's signature scheme.

==> macro.tex <==
%Raccourcis
\let\ds\mathds

\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern.1pt\mathchar"0362\kern.1pt}%
    {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
  }{\textheight}% 
}{2.4ex}}%
\stackon[-6.9pt]{#1}{\tmpbox}%
}
%Notations quantiques
%\newcommand{\norm}[1]{\left|\!\left| #1 \right|\!\right|}
\newcommand{\QFT}[1]{\reallywidehat{\ket{#1}}}

%Notations italiques
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
%\newcommand{\cS}{\mathcal{S}}

%Notations double barre
%\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zq}{\Z_q}
\newcommand{\Fq}{\F_q}

%Intervalle
\newcommand{\interv}{[\![-\frac{q-1}{2},\frac{q-1}{2}]\!]}
\newcommand{\interval}[2]{\left[\!\!\left[#1,#2\right]\!\!\right]}
%Code
\newcommand{\CC}{\ensuremath{\mathscr{C}}}

%\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\algo}[1]{\mathcal{#1}}
\newcommand{\set}[1]{\mathcal{#1}}

%lettres calligraphiques
\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Dc}{{\pazocal D}}
\newcommand{\Ec}{{\pazocal E}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Xc}{{\mathcal X}}

%Vecteurs
\newcommand{\av}{\vec{a}}
\newcommand{\bv}{\vec{b}}
\newcommand{\cv}{\vec{c}}
\renewcommand{\dv}{\vec{d}}
\renewcommand{\ev}{\vec{e}}
\newcommand{\sv}{\vec{s}}
\newcommand{\tv}{\vec{t}}
\newcommand{\uv}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\wv}{\vec{w}}
\newcommand{\xv}{\vec{x}}
\newcommand{\yv}{\vec{y}}
\newcommand{\zv}{\vec{z}}
\newcommand{\zero}[1]{\vec{0}_{#1}}
\newcommand{\un}{\vec{1}}
\newcommand{\und}{\mathds{1}}

%Matrices
\newcommand{\Am}{\vec{A}}
\newcommand{\Bm}{\vec{B}}
\newcommand{\Cm}{\vec{C}}
\newcommand{\Dm}{\vec{D}}
\newcommand{\Em}{\vec{E}}
\newcommand{\Fm}{\vec{F}}
\newcommand{\Gm}{\vec{G}}
\newcommand{\Hm}{\vec{H}}
\newcommand{\Mm}{\vec{M}}
\newcommand{\Nm}{\vec{N}}
\newcommand{\Pm}{\vec{P}}
\newcommand{\Rm}{\vec{R}}
\newcommand{\Sm}{\vec{S}}
\newcommand{\Tm}{\vec{T}}
\newcommand{\Um}{\vec{U}}
\newcommand{\Xm}{\vec{X}}
\newcommand{\Ym}{\vec{Y}}
\newcommand{\Zm}{\vec{Z}}
\newcommand{\Had}[2]{\mat{H}_{#1,#2}} % Hadamard gate
\newcommand{\Id}{\vec{Id}}

%Probabilites
\newcommand{\esp}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\prob}{\pi_{\ev}}
\newcommand{\probdual}{\hat{\pi}_{\cv^\perp}}

%Sommes
\newcommand{\subV}{\substack{V \le \Fq^m \\ \dim V = t}}
\newcommand{\sumV}{\sum_{\subV}}
\newcommand{\sumW}{\sum_{\substack{W \le \Fq^m \\ \dim W = t \\ W \neq V}}}
\newcommand{\subyt}{\substack{\vec{y} \in \Fq^n \\ \wt{y} = t}}
\newcommand{\sumyt}{\sum_{\subyt}}

\newcommand{\sumFq}[1]{\sum_{#1 \in \Fq^\ast}}
\newcommand{\sumFqn}[1]{\sum_{\vec{#1} \in \Fq^n}}
\newcommand{\sumcode}{\sum_{\cv \in \CC}}
\newcommand{\sumdual}{\sum_{\cv^\perp \in \CC^\perp}}

%Valeurs entieres superieure et inferieure
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%Coefficients gaussiens
\newcommand{\gauss}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

%Produit scalaire
\newcommand{\innerprod}[2]{\vec{#1} \cdot \vec{#2}}

%Poids et distances
\newcommand\wt[1]{\abs{\vec{#1}}}
\newcommand{\dr}{d_{\textup{rank}}}
\newcommand\wtr[1]{\abs{\vec{#1}}_{\textup{rank}}}
\newcommand\wth[1]{\abs{\vec{#1}}_{\textup{Ham}}}
\newcommand\wtl[1]{\abs{\vec{#1}}_{\textup{Lee}}}
\newcommand\dl{d_{\textup{Lee}}}
\newcommand{\weasy}{w_{\textup{easy}}}
\newcommand{\omeasy}{\omega_{\textup{easy}}}

%Distances
\newcommand{\dgv}{d_{\textup{GV}}}
\newcommand{\drgv}{\tau_{\textup{GV}}}
\newcommand{\dmin}{d_{\textup{min}}}
\newcommand{\dtr}{D_{\textup{tr}}}
\newcommand{\dstat}{D_{\textup{stat}}}

%etats intermediaires de la reduction
\newcommand{\psiA}{\ket{\psi_{\Ac}}}
\newcommand{\psiAQFT}{\ket{\psi_{\Ac}^{\textup{QFT}}}}
\newcommand{\psiideal}{\ket{\psi_{\text{ideal}}}}
\newcommand{\psiidealQFT}{\ket{\psi_{\text{ideal}}^{\textup{QFT}}}}
\newcommand{\psiAs}{\psi_{\Ac}}
\newcommand{\psiideals}{\psi_{\text{ideal}}}

%Trace
\newcommand{\Trac}[2]{\textup{Tr}_{#1 / #2}}

%operateurs mathematiques
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\rank}{Rank}

% \OO{ } : grand O de { }
\newcommand{\OOtsp}[1]{O(#1)} % OO textstyle parentheses --> to be preferred to avoid vertical space ugliness
\newcommand{\Thtsp}[1]{\Theta(#1)} % Theta textstyle parentheses --> to be preferred to avoid vertical space ugliness
\newcommand{\OO}[1]{O\left( #1 \right)}
\newcommand{\Th}[1]{\Theta\left( #1 \right)}
\newcommand{\Tht}[1]{\tilde{\Theta}\left( #1 \right)}
\newcommand{\OOt}[1]{\tilde{O}\left( #1 \right)}
\newcommand{\Om}[1]{\Omega \left( #1 \right)}
\newcommand{\Omt}[1]{\tilde{\Omega} \left( #1 \right)}

%Transposition
\makeatletter
\newcommand*{\transp}{{\mathpalette\@transpose{}}}
\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
\makeatother
\newcommand{\transpose}[1]{{#1}^{\transp}}
\newcommand{\tran}[1]{\transpose{#1}}

%Def equal
\newcommand*{\eqdef}{\stackrel{\text{def}}{=}}

%Probleme 
\newcommand{\sdecP}{\textup{$\mathsf{SDP}$}}
\newcommand{\SDP}{\sdecP}
\newcommand{\scodeP}{\textup{$\mathsf{SCP}$}}
\newcommand{\SCP}{\scodeP}
%JP: je mets des macros supplémentaires, je ne comprends pas la logique de ces abréviations et je suis incapable de m'en souvenir quand je les ecris.

%Environnement 
\newtheorem{definition}{Definition}
%\newtheorem{problem}{Problem}
\newtheorem{notation}{Notation}
\newtheorem{fact}{Fact}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumption}{Assumption}
\newtheorem{rthumb}{Rule of thumb}

%Style
\renewcommand{\thefootnote}{\texttt{(\arabic{footnote})}} % Numéros des notes de bas de page plus lisibles
\renewcommand{\baselinestretch}{1.1} % Espacement des lignes
\sloppy % Espacement des mots plutôt que césure
\setlength{\parindent}{0pt} % Empêcher les alinéas
\setlength{\parskip}{3pt} % Espacement des paragraphes
\renewcommand*\thesection{\arabic{section}}

%commandes pour les commentaires
\newcommand{\jp}[1]{{\textcolor{red}{JP: #1}}}
\newcommand{\andre}[1]{{\color{blue} André: #1 \color{black}}}
\newcommand{\simona}[1]{{\color{blue} Simona: #1 \color{black}}}
\newcommand{\toto}[1]{{\color{green} Toto: #1 \color{black}}}

%André
\newcommand{\zo}{\{0,1\}}

%<<<<<<< HEAD
%\newtheorem{assumption}{Assumption}
%=======
%>>>>>>> 290ea4bbd9c9ade0af00bc789a69c3012d760d39
%<<<<<<< HEAD
%
%=======
%>>>>>>> 7be7f12c04722a9a453421ba8af42f07d1355d5d

% FOR HAVING SEVERAL KEYS FOR THE SAME BIBLIOGRAPHIC ENTRY

 \makeatletter
% \bibalias{<alias>}{<source>} makes \cite{<alias>} equivalent to \cite{<source>}
\newcommand\bibalias[2]{%
  \@namedef{bibali@#1}{#2}%
}

\newtoks\biba@toks
\newcommand\acite[2][]{%
  \biba@toks{\cite#1}%
  \def\biba@comma{}%
  \def\biba@all{}%
  \@for\biba@one:=#2\do{%
    \@ifundefined{bibali@\biba@one}{%
      \edef\biba@all{\biba@all\biba@comma\biba@one}%
    }{%
      \PackageInfo{bibalias}{%
        Replacing citation `\biba@one' with `\@nameuse{bibali@\biba@one}'
      }%
      \edef\biba@all{\biba@all\biba@comma\@nameuse{bibali@\biba@one}}%
    }%
    \def\biba@comma{,}%
  }%
  \edef\biba@tmp{\the\biba@toks{\biba@all}}%
  \biba@tmp
}
\makeatother

\bibalias{Ouroboros-R}{AABBBDGHZ17}
\bibalias{RQC}{AABBBDGZ17}
\bibalias{RQC2}{AABBBDGZCH19}
\bibalias{ROLLO}{ABDGHRTZABBBO19}
\bibalias{LAKE}{ABDGHRTZ17}
\bibalias{LOCKER}{ABDGHRTZ17a}
\bibalias{RankSign}{AGHRZ17}

